Words or Vision: Do Vision-Language Models Have Blind Faith in Text?

Vision-Language Models (VLMs) excel in integrating visual and textual information for vision-centric tasks, but their handling of inconsistencies between modalities is underexplored. We investigate VLMs' modality preferences when faced with visual data and varied textual inputs in vision-centered settings. By introducing textual variations to four vision-centric tasks and evaluating ten Vision-Language Models (VLMs), we discover a \emph{``blind faith in text''} phenomenon: VLMs disproportionately trust textual data over visual data when inconsistencies arise, leading to significant performance drops under corrupted text and raising safety concerns. We analyze factors influencing this text bias, including instruction prompts, language model size, text relevance, token order, and the interplay between visual and textual certainty. While certain factors, such as scaling up the language model size, slightly mitigate text bias, others like token order can exacerbate it due to positional biases inherited from language models. To address this issue, we explore supervised fine-tuning with text augmentation and demonstrate its effectiveness in reducing text bias. Additionally, we provide a theoretical analysis suggesting that the blind faith in text phenomenon may stem from an imbalance of pure text and multi-modal data during training. Our findings highlight the need for balanced training and careful consideration of modality interactions in VLMs to enhance their robustness and reliability in handling multi-modal data inconsistencies.

==> tables/app_text_only_acc.tex <==
\begin{table}[htbp]
    \centering
    \small
    \scalebox{0.9}{
    \begin{tabular}{lcccc}
        \toprule
        & \multicolumn{4}{c}{VQAv2 (Text-only)} \\
        \cmidrule(lr){2-5}
        Model & Base & Match & Corruption & Irrelevance \\
        \midrule
        Molmo-7B-D & 76.33 & 88.98 & 18.74 & 35.40 \\
        claude-3-5-sonnet & 66.88 & 84.39 & 16.17 & 24.39 \\
        GPT-4o & 78.39 & 90.07 & 17.59 & 18.67 \\
        GPT-4o-mini & 69.82 & 90.19 & 17.34 & 21.35 \\
        llava-v1.6-vicuna-7b & 79.45 & 92.82 & 18.32 & 38.70 \\
        llava-1.5-13b & 77.76 & 92.78 & 18.56 & 36.70 \\
        llava-1.5-7b & 75.56 & 92.69 & 18.45 & 38.57 \\
        llava-v1.6-vicuna-13b & 81.02 & 92.96 & 18.58 & 37.60 \\
        Phi3.5 & 75.65 & 91.06 & 18.41 & 34.32 \\
        \bottomrule
    \end{tabular}}
    \caption{Text-only Performance (\%) across different models. It provides a sanity check for the constructed text when matched, corrupted, or irrelevant.}
    \label{tab:benchmark}
\end{table}


==> tables/benchmark.tex <==



\begin{table}[htbp]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.0}
    % \resizebox{0.8\textwidth}{!}{
    \footnotesize
    \scalebox{0.95}{
    \begin{tabular}{lccccc}
        \toprule
        & \multicolumn{5}{c}{VQAv2} \\
        \cmidrule(lr){2-6}
      
        Model & \makecell{Base \\ ($X_{\textsc{i}}$)} & \makecell{Match \\ ($X_{\textsc{i}}+X_{\textsc{t}}^m$)} & \makecell{Corruption \\ ($X_{\textsc{i}}+X_{\textsc{t}}^c$)} & \makecell{Irrelevance \\ ($X_{\textsc{i}}+X_{\textsc{t}}^\text{irr}$)} & \makecell{Avg \\ ($X_{\textsc{i}}+X_{\textsc{t}}$)} \\
        \midrule
      

        Claude Haiku & 50.08 & 83.40 & 25.54 & 48.55 & 52.50 \\
        Claude Sonnet & 66.88 & 77.85 & 68.17 & 70.89 & 72.30 \\
        GPT-4o mini & 69.82 & 87.49 & 51.55 & 72.11 & 70.38 \\
        GPT-4o & 78.39 & 89.27 & \textbf{70.75} & 78.82 & \textbf{79.61} \\
        \hdashline[0.5pt/2pt]
        LLaVA-1.5-7B & 75.56 & 92.21 & 30.58 & 75.27 & 66.02 \\
        LLaVA-1.5-13B & 77.76 & 92.84 & 36.05 & 78.01 & 68.97 \\
        LLaVA-NeXT-7B & 79.45 & 92.32 & 28.69 & 79.43 & 66.81 \\
        LLaVA-NeXT-13B & 81.02 & \textbf{93.59} & 37.61 & 81.29 & 70.83 \\
        LLaVA-NeXT-34B & 82.96 & 93.07 & 42.87 & 79.64 & 71.86 \\

        Phi3.5 & 75.65 & 91.23 & 35.23 & 74.87 & 67.11 \\
        Molmo-7B-D & 76.33 & 88.57 & 49.29 & 76.50 & 71.45 \\
        Qwen2-VL-7B & \textbf{85.51} & 92.76 & 50.79 & \textbf{83.70} & 75.75 \\


        \midrule
        & \multicolumn{5}{c}{DocVQA} \\
        \cmidrule(lr){2-6}
       
        Model & \makecell{Base \\ ($X_{\textsc{i}}$)} & \makecell{Match \\ ($X_{\textsc{i}}+X_{\textsc{t}}^m$)} & \makecell{Corruption \\ ($X_{\textsc{i}}+X_{\textsc{t}}^c$)} & \makecell{Irrelevance \\ ($X_{\textsc{i}}+X_{\textsc{t}}^\text{irr}$)} & \makecell{Avg \\ ($X_{\textsc{i}}+X_{\textsc{t}}$)} \\
        \midrule
       
        Claude Haiku & 68.80 & 81.60 & 40.20 & 56.00 & 59.27 \\
        Claude Sonnet & 87.00 & 91.20 & \textbf{84.60} & 87.20 & \textbf{87.67} \\
        GPT-4o mini & 69.40 & 81.40 & 38.20 & 67.20 & 62.27 \\
        GPT-4o & 85.00 & 90.40 & 73.60 & 86.40 & 83.47 \\
        \hdashline[0.5pt/2pt]
        % \midrule
        LLaVA-1.5-7B & 14.50 & 85.90 & 3.60 & 13.40 & 34.30 \\
        LLaVA-1.5-13B & 16.00 & 86.30 & 3.70 & 15.90 & 35.30 \\
        LLaVA-NeXT-7B & 53.60 & 90.80 & 10.00 & 52.40 & 51.07 \\
        LLaVA-NeXT-13B & 57.70 & 90.40 & 11.00 & 55.80 & 52.40 \\
        LLaVA-NeXT-34B & 64.00 & 87.80 & 15.10 & 62.70 & 55.20 \\

        Phi3.5 & 78.20 & 92.40 & 50.50 & 77.00 & 73.30 \\
        Molmo-7B-D & 74.00 & 90.30 & 38.40 & 74.70 & 67.80 \\
        Qwen2-VL-7B & \textbf{90.50} & \textbf{95.10} & 57.50 & \textbf{89.90} & 80.83 \\

        % \bottomrule
                        \midrule
        & \multicolumn{5}{c}{MathVista} \\
        \cmidrule(lr){2-6}
        Model & \makecell{Base \\ ($X_{\textsc{i}}$)} & \makecell{Match \\ ($X_{\textsc{i}}+X_{\textsc{t}}^m$)} & \makecell{Corruption \\ ($X_{\textsc{i}}+X_{\textsc{t}}^c$)} & \makecell{Irrelevance \\ ($X_{\textsc{i}}+X_{\textsc{t}}^\text{irr}$)} & \makecell{Avg \\ ($X_{\textsc{i}}+X_{\textsc{t}}$)} \\
        \midrule
        Claude Haiku &41.00 & 80.30 & 19.80 & 39.70 & 46.60 \\
        Claude Sonnet &56.30 & 68.10 & 49.30 & 55.20 & 57.53   \\
        GPT-4o mini & 52.30 & 73.80 & 23.90 & 44.40 & 47.37 \\
        GPT-4o & 58.90 & 73.70 & 41.20 & 53.10 & 56.00 \\
        \hdashline[0.5pt/2pt]
        LLaVA-1.5-7B & 27.30 & 74.80 & 19.30 & 28.40 & 40.83 \\
        LLaVA-1.5-13B & 29.60 & 76.20 & 19.40 & 28.50 & 41.37 \\
        LLaVA-NeXT-7B &35.80 & 71.80 & 19.70 & 31.60 & 41.03 \\
        LLaVA-NeXT-13B & 36.20 & 73.10 & 20.60 & 32.60 & 42.10 \\
        LLaVA-NeXT-34B &  34.00	& 68.00 & 21.70 & 32.10 & 40.60  \\

        Phi3.5 & 43.10 & 73.70 & 22.20 & 41.10 & 45.67 \\
        Molmo-7B-D & 44.90 & 68.50 & 32.90 & 45.30 & 48.90 \\
                Qwen2-VL-7B &  55.40 & 	77.80 & 28.90 & 54.90 & 53.87\\
       
        

        \bottomrule
    \end{tabular}}
    \caption{Performance}
    \label{tab:benchmark}
\end{table}


==> tables/brand_detect.tex <==



\begin{table}[htbp]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.0}
    % \resizebox{0.8\textwidth}{!}{
    \footnotesize
    \scalebox{0.95}{
    \begin{tabular}{l|ccccc}
        \hline
        & \multicolumn{5}{c}{\textbf{Brand Recognition}} \\
      
        Model & Base $\uparrow$ & Match $\uparrow$ & Corruption $\uparrow$ & Irrelevance $\uparrow$ & Marco $\uparrow$ \\
        \hline
        GPT-4o mini & 88.84&86.88&84.8&88.48&86.72 \\
        Claude Haiku &84.40&83.40&78.72&82.28&81.47   \\
        GPT-4o & 88.68&89.48&89.76&89.16&89.47 \\
        Claude Sonnet &\textbf{90.20}&\textbf{90.56}&\textbf{90.24}&\textbf{90.24}&\textbf{90.35}   \\

        \hdashline[0.5pt/2pt]
        LLaVA-1.5-7B & 57.28&77.56&62.52&16.28&52.12 \\
        LLaVA-1.5-13B & 61.20&79.00&33.96&11.72&41.56 \\
        LLaVA-NeXT-7B & 78.60&77.40&55.32&6.60&46.44 \\
        LLaVA-NeXT-13B & 83.00&82.56&60.00&23.20&55.25 \\
        LLaVA-NeXT-34B & 66.28 & 68.28 & 53.52 & 52.84 & 58.21  \\

        Phi3.5 & 84.40&83.84&60.68&16.44&53.65 \\
        Molmo-7B-D & 87.44&87.32&41.44&60.88&63.21 \\
        Qwen2-VL-7B &  89.68 & 88.92 & 86.48 & 70.16 & 81.85\\
        \hline
    \end{tabular}}
    \caption{Performance}
    \label{tab:brand_detect}
\end{table}


==> tables/data_ablation.tex <==
\begin{table}[htbp]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    % \renewcommand{\arraystretch}{1.0}
    % \resizebox{0.8\textwidth}{!}{
    \footnotesize
    \scalebox{0.95}{
    \begin{tabular}{lccccc}
        \toprule
        & \multicolumn{5}{c}{VQAv2} \\
        \cmidrule(lr){2-6}

        Model & \makecell{Base \\ ($X_{\textsc{i}}$)} & \makecell{Match \\ ($X_{\textsc{i}}+X_{\textsc{t}}^m$)} & \makecell{Corruption \\ ($X_{\textsc{i}}+X_{\textsc{t}}^c$)} & \makecell{Irrelevance \\ ($X_{\textsc{i}}+X_{\textsc{t}}^\text{irr}$)} & \makecell{Avg \\ ($X_{\textsc{i}}+X_{\textsc{t}}$)} \\
        \midrule
        
        LLaVA-v1.6-7B & \textbf{79.45} & \textbf{92.32} & 28.69 & \textbf{79.43} & 66.81 \\
        \midrule
        SFT & 77.48 & 87.56 & 71.25 & 77.32 & 78.71 \\
        wo/ text-only data & 77.81 & 83.98 & 75.26 & 77.40 & \textbf{78.88} \\
        
      
        
        \bottomrule
    \end{tabular}}
    \caption{In-distribution performance comparison between original models and fine-tuned models.}
    \label{tab:ft_res}
\end{table}


==> tables/order_effect.tex <==

\begin{table*}[ht]
    \centering
    \begin{tabular}{lccc}
        \hline
        Order& Match & Corruption & Irrelevance \\
        \hline
        $<$image$>$ first, $<$textual information$>$ later & 79.51 & 74.05 & 2.25 \\
        $<$textual information$>$ first, $<$image$>$ later & 82.21 & 79.51 & 18.49 \\
        \hline
    \end{tabular}
    \caption{Text Ratio (\%) with different token orders under different text conditions for \texttt{Phi3.5}. We provide the complete examples in the appendix.}
    \label{tab:order_effect}
\end{table*}


==> tables/prompt_effect.tex <==

\begin{table*}[h]
    \centering
    \begin{tabular}{lccc}
        \hline
        Prompt & Match & Corruption & Irrelevance \\
        \hline
        $<$question$>$ & 88.32 & 59.40 & 9.36 \\
        Please focus on the image to answer the question: $<$question$>$ & 84.87 & 45.49 & 9.63 \\
        Please focus on the textual information to answer the question: $<$question$>$ & 87.91 & 64.78 & 10.66 \\
        \hline
        Avg & 86.98 & 56.56 & 9.88 \\
        \hline
    \end{tabular}
    \caption{Text ratio (\%) across different prompts and text conditions for \texttt{Molmo-7B-D}. Instructional prompts can adjust the model’s focus between modalities, but a strong text preference remains (over 50\% on average with corrupted text). Full examples are provided in the appendix. }
    \label{tab:prompt_effect}

\end{table*}


